Design and Analysis of Bipartite Experiments under a Linear Exposure-Response Model

A bipartite experiment consists of one set of units being assigned treatments and another set of units for which we measure outcomes. The two sets of units are connected by a bipartite graph, governing how the treated units can affect the outcome units. In this paper, we consider estimation of the average total treatment effect in the bipartite experimental framework under a linear exposure-response model. We introduce the Exposure Reweighted Linear (ERL) estimator, and show that the estimator is unbiased, consistent and asymptotically normal, provided that the bipartite graph is sufficiently sparse. To facilitate inference, we introduce an unbiased and consistent estimator of the variance of the ERL point estimator. In addition, we introduce a cluster-based design, Exposure-Design, that uses heuristics to increase the precision of the ERL estimator by realizing a desirable exposure distribution.

==> old-tex/app-intervals.tex <==
\section{Variance Estimation}\label{sec:interval-proofs}

In this section, we prove Lemmas~\ref{lem:variance-terms} and \ref{lem:covariance-terms}, which are then used to prove Theorem~\ref{thm:variance-estimate}, which establishes unbiasedness of the proposed variance estimator.

% First, we show Lemma~\ref{lem:variance-terms}, which demonstrates how to estimate the variance of an individual treatment effect estimate.
% To do so, we need to decompose the random variable $Q_i$.
% For each outcome unit $i \in \outunits$, define the random variable $T_i$ to be the second term in the function $Q_i$. 
% That is,
% \[
% T_i = 
% \frac{\Var{\dosei} \paren{\dosei^2 - \Exp{\dosei^2}} - \Cov{\dosei, \dosei^2} \paren{\dosei - \Exp{\dosei}}  }{\Var{\dosei} \Var{\dosei^2} - \Cov{\dosei, \dosei^2}^2}
% \]
% so that $Q_i \triangleq \frac{\paren{\dosei - \Exp{\dosei}}^2}{\Var{\dosei}^2} - T_i$.
% The following Lemma states the key properties of the random variable $T_i$, and consequently $Q_i$, which allow for the proof of Lemma~\ref{lem:variance-terms}.

% \begin{lemma}\label{lem:properties-of-T}
% If the exposure $\dosei$ takes at least three values with non-zero probability, then the function $T_i$ satisfies the following three properties:
% \begin{itemize}
%     \item $\Exp{T_i} = 0$
%     \item $\Exp{\dosei T_i} = 0$
%     \item $\Exp{\dosei^2 T_i} = 1$
% \end{itemize}
% \end{lemma}
% \begin{proof}
% For notational simplicity, we drop the subscript as write $\dosei$ as $x$ and $T_i$ as $T$.

% First, we will show that the denominator $\Var{x}\Var{x^2} - \Cov{x,x^2}^2$ is positive when the exposure $x$ takes at least three values with non-zero probability.
% By Cauchy-Schwarz, we have that $\Cov{x,x^2}^2 \leq \Var{x}\Var{x^2}$, which establishes that denominator is non-negative.
% The Cauchy-Schwarz inequality is strict precisely when $x$ and $x^2$ are not perfectly correlated, i.e. there does not exist $a$ and $b$ such that $x^2 = a x + b$.
% Note that this cannot happen when $x$ takes three distinct values.
% Thus, the Cauchy-Schwarz is strict in this case so that the denominator is positive.
% For notational convenience, we write the denominator as $\Delta = \Var{x}\Var{x^2} - \Cov{x,x^2}^2$ throughout the remainder of the proof.

% We will now show the three properties.
% The first property follows by linearity of expectation, as
% \begin{align*}
%     \Delta \cdot \Exp{T}
%     &= \Exp{ \Var{\dosei} \paren{x^2 - \Exp{x^2}} - \Cov{x, x^2} \paren{x - \Exp{x}} } \\
%     &= \Var{x} \paren{\Exp{x^2} - \Exp{x^2}} - \Cov{x, x^2} \paren{\Exp{x} - \Exp{x}} \\
%     &= 0 \enspace,
% \end{align*}
% and the result follows by dividing through by $\Delta$ on both sides.
% Next, we show the second property.
% Again, by linearity of expectation, we have that
% \begin{align*}
%     \Delta \cdot \Exp{x T}
%     &= \Exp{ \Var{\dosei} \paren{x^3 - x\Exp{x^2}} - \Cov{x, x^2} \paren{x^2 - x\Exp{x}} } \\
%     &= \Var{x} \paren{\Exp{x^3} - \Exp{x}\Exp{x^2}} - \Cov{x, x^2} \paren{\Exp{x^2} - \Exp{x}^2} \\
%     &= \Var{x} \Cov{x, x^2} - \Cov{x, x^2} \Var{x} \\
%     &= 0 \enspace,
% \end{align*}
% and the result follows by dividing through by $\Delta$ on both sides.
% Finally, we show the third property.
% By linearity of expectation, 
% \begin{align*}
%     \Delta \cdot \Exp{x^2 T}
%     &= \Exp{ \Var{\dosei} \paren{x^4 - x^2 \Exp{x^2}} - \Cov{x, x^2} \paren{x^3 - x^2\Exp{x}}} \\
%     &= \Var{x} \paren{\Exp{x^4} - \Exp{x^2}^2} - \Cov{x, x^2} \paren{\Exp{x^3} - \Exp{x^2}\Exp{x}} \\
%     &= \Var{x} \Var{x^2} - \Cov{x, x^2}^2 \\
%     &= \Delta \enspace,
% \end{align*}
% and the result follows by dividing both sides by $\Delta$.
% \end{proof}

% We are now ready to prove Lemma~\ref{lem:variance-terms}, which we restate here.
% \begin{manuallemma}{\ref{lem:variance-terms}}
% \variancetermlemma
% \end{manuallemma}
% \begin{proof}
% We may use the properties of the random variable $T_i$ proved in Lemma~\ref{lem:properties-of-T} together with the linear response assumption to obtain
% \begin{align*}
%     \Exp[\Big]{\poi(\zv)^2 T_i}
%     &= \Exp[\Big]{\paren{\slopei \dosei + \incepti}^2 T_i}
%         &\text{(linear response)} \\
%     &= \slopei^2 \Exp[\Big]{\dosei^2 T_i} + 2 \slopei \incepti \Exp[\Big]{\dosei T_i} + \incepti^2 \Exp[\Big]{T_i} 
%         &\text{(expanding terms)} \\
%     &= \slopei^2 .
%         &\text{(Lemma~\ref{lem:properties-of-T})}
% \end{align*}
% Next, we write the variance of individual treatment effect estimator.
% Because the individual treatment effect estimator is unbiased,
% \begin{align*}
%     \Var{\dhtesti}
%     &= \Exp{\dhtesti^2} - \Exp{\dhtesti}^2 \\
%     &= 4 \cdot \Exp[\Big]{ \poi(\zv)^2 \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}}^2 } - 4 \cdot \slopei^2 \\
%     &= 4 \cdot \Exp[\Big]{ \poi(\zv)^2 \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}}^2 } - 4 \cdot \Exp[\Big]{\poi(\zv)^2 T_i} \\
%     &= 4 \cdot \Exp[\Big]{ \poi(\zv)^2 \bracket[\Big]{\paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}}^2 - T_i } } \\
%     &= 4 \cdot \Exp{\poi(\zv)^2 Q_i} \enspace.
% \end{align*}
% \end{proof}


% Next, we will prove Lemma~\ref{lem:covariance-terms} which demonstrates how to estimate the covariance between two individual treatment effects.
% To do so, we need to decompose the random variable $R_{i,j}$.
% For each pair of outcome units $i,j \in \outunits$, define the random variable $S_{i,j}$ to be the second term in the random variable $R_{i,j}$. 
% That is,
% \[
% S_{i,j} =
% \frac{a_{i,j} \paren{\dosei \dosej - \Exp{\dosei \dosej}} + b_{i,j} \paren{\dosei - \Exp{\dosei}} + c_{i,j} \paren{\dosej - \Exp{\dosej}} }{\Psi_{i,j}} \enspace,
% \]
% where we recall that these coefficients are given as 
% $a_{i,j},b_{i,j},c_{i,j},\Psi_{i,j}$ are defined as 
% \begin{align*}
% a_{i,j} & = \Var{\dosei} \Var{\dosej} - \Cov{\dosei,\dosej}^2 \\
% b_{i,j} & = \Cov{\dosei,\dosej} \Cov{ \dosei \dosej, \dosej} - \Var{\dosej} \Cov{\dosei \dosej, \dosei}\\
% c_{i,j} & = \Cov{\dosei,\dosej} \Cov{ \dosei \dosej, \dosei} -  \Var{\dosei} \Cov{\dosei \dosej, \dosej}\\
% \Psi_{i,j} &= \Var{\dosei \dosej} \paren{ \Var{\dosei}\Var{\dosej} - \Cov{\dosei, \dosej}^2} \\
%     &\quad - \Var{\dosei} \Cov{\dosei \dosej, \dosej}^2 
%     - \Var{\dosej} \Cov{\dosei \dosej, \dosei}^2 
%     + 2 \Cov{\dosei, \dosej} \Cov{\dosei \dosej,\dosej} \Cov{\dosei \dosej, \dosei}  \enspace.
% \end{align*}
% In this way, $R_{i,j} \triangleq \paren{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} - S_{i,j}$.
% The following lemma states the key properties of the random variable $S_{i,j}$, and consequently $R_{i,j}$, which allow for the proof of Lemma~\ref{lem:covariance-terms}.

% \begin{lemma}\label{lem:properties-of-S}
% Fix a pair of outcome units $i,j \in \outunits$. 
% If $\Psi_{i,j} \neq 0$, then the random variable $S_{i,j}$ satisfies the following properties:
% \begin{itemize}
%     \item $\Exp{S_{i,j}} = 0$
%     \item $\Exp{\dosei S_{i,j}} = \Exp{\dosej S_{i,j}} = 0$
%     \item $\Exp{\dosei \dosej S_{i,j}} = 1$
% \end{itemize}
% \end{lemma}
% \begin{proof}
% For notational simplicity, we will drop the subscripts and write $\dosei$ as $x$, $\dosej$ as $y$ and $S_{i,j}$ as $S$.
% In the same way, we will write $a_{i,j}, b_{i,j}, c_{i,j}$, and $\Psi_{i,j}$ as $a,b,c$, and $\Psi$.

% Given that $\Psi > 0$, we seek to verify the three properties in the lemma.
% The first is easy to verify by the linearity of expectation, as
% \begin{align*}
% \Psi \cdot \Exp{S} 
% &= \Exp{ a(xy - \Exp{xy}) + b (x - \Exp{x}) + c (y - \Exp{y}) } \\
% &= a ( \Exp{xy} - \Exp{xy} ) + b (\Exp{x} - \Exp{x}) + c (\Exp{y} - \Exp{y} \\
% &= 0 
% \end{align*}
% so that dividing both sides by $\Psi$ yields the desired result.
% We now verify the second property.
% Observe that
% \begin{align*}
% \Psi \cdot \Exp{x S} 
% &= a \cdot ( \Exp{x^2 y} - \Exp{x}\Exp{xy}) + b \cdot (\Exp{x^2} - \Exp{x}^2) + c \cdot (\Exp{xy} - \Exp{x}\Exp{y}) \\
% &= a \cdot \Cov{xy,x} + b \cdot \Var{x} + c \cdot \Cov{x,y} \\
% &= \Cov{xy,x} (\Var{x} \Var{y} - \Cov{x,y}^2) \\
% &\quad\quad+ \Var{x} (\Cov{x,y} \Cov{xy,y} - \Var{y} \Cov{xy,x}) \\
% &\quad\quad + \Cov{x,y}(\Cov{x,y} \Cov{xy,x} - \Var{x} \Cov{xy,y}) \\
% &= 0 \enspace,
% \end{align*}
% and dividing both sides by $\Psi$ yields the desired result.
% The proof that $\Exp{y S(x,y)} = 0$ follows in exactly the same fashion.
% Finally, we verify the third property.
% Observe that
% \begin{align*}
% \Psi \cdot \Exp{x y S} 
% &= a \cdot ( \Exp{(xy)^2} - \Exp{xy}^2) + b \cdot (\Exp{x^2y} - \Exp{xy} \Exp{x}) + c \cdot (\Exp{xy^2} - \Exp{xy} \Exp{y}) \\
% &= a \cdot \Var{xy} + b \cdot \Cov{xy,x} + c \cdot \Cov{xy,y} \\
% &= \Var{xy} (\Var{x} \Var{y} - \Cov{x,y}^2) \\
% &\quad\quad+ \Cov{xy,x} (\Cov{x,y} \Cov{xy,y} - \Var{y} \Cov{xy,x}) \\
% &\quad\quad + \Cov{xy,y}(\Cov{x,y} \Cov{xy,x} - \Var{x} \Cov{xy,y} ) \\
% &= \Var{xy} (\Var{x} \Var{y} - \Cov{x,y}^2) \\
% &\quad\quad - \Var{x} \Cov{xy,y}^2 - \Var{y} \Cov{xy,x}^2  \\
% &\quad\quad + 2 \Cov{x,y} \Cov{xy,y} \Cov{xy,x} \\
% &= \Psi \enspace,
% \end{align*}
% so that dividing both sides by $\Psi$ yields the desired result.
% \end{proof}

% Finally, we are ready to prove Lemma~\ref{lem:covariance-terms}, which is the last result needed to establish that the variance estimator is unbiased.
% We restate the lemma below.
% \begin{manuallemma}{\ref{lem:covariance-terms}}
% \covariancetermlemma
% \end{manuallemma}

\begin{proof}
We may use the properties of the random variable $S_{i,j}$ proved in Lemma~\ref{lem:properties-of-S} together with the linear response assumption to obtain
\begin{align*}
\Exp{ \poi(\zv) \poj(\zv) S_{i,j} }
&= \Exp{ (\slopei \dosei + \incepti) (\slopej \dosej + \inceptj) S_{i,j}} 
    &\text{(linear response)}\\
&= \slopei \slopej\Exp{\dosei \dosej S_{i,j}} + \incepti \inceptj \Exp{S_{i,j}} + \slopei \inceptj \Exp{ \dosei S_{i,j} } + \slopej \incepti \Exp{ \dosej S_{i,j} } 
    &\text{(expanding terms)}\\
&= \slopei \slopej
    \enspace.
    &\text{(Lemma~\ref{lem:properties-of-S})} 
\end{align*}
Next, we write the covariance between the individual treatment effect estimators.
Because the individual treatment effect estimators are unbiased,
\begin{align*}
\Cov{\dhtesti, \dhtestj} 
&= \Exp{\dhtesti \dhtestj} - \Exp{\dhtesti} \Exp{\dhtestj} \\
&= \Exp{\dhtesti \dhtestj} - \itei \itej \\
&= 4 \cdot \Exp[\Big]{\poi(\zv) \poj(\zv) \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} }
- 4 \cdot \slopei \slopej \\
&= 4 \cdot \Exp[\Big]{\poi(\zv) \poj(\zv) \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} }
- 4 \cdot \Exp{ \poi(\zv) \poj(\zv) S_{i,j} } \\
&= 4 \cdot \Exp[\Big]{ \poi(\zv) \poj(\zv) \bracket[\Big]{\paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} - S_{i,j}} } \\
&= 4 \cdot \Exp[\Big]{ \poi(\zv) \poj(\zv) R_{i,j} }
\qedhere
\end{align*}
\end{proof}

We are now ready to prove Theorem~\ref{thm:variance-estimate}, which establishes unbiasedness of the variance estimator.
\begin{manualtheorem}{\ref{thm:variance-estimate}}
\varestthm
\end{manualtheorem}

\begin{proof}
We may calculate the expectation of the variance estimate $\erlvarest$ as
\begin{align*}
\Exp{\erlvarest} 
&= \Exp[\Bigg]{
\frac{4}{n^2} \sum_{i=1}^n \bracket[\Big]{  \poi(\zv)^2 Q_i
 + \sum_{j \neq i} \poi(\zv) \poj(\zv) R_{i,j}} 
} \\
&= \frac{1}{n^2} \sum_{i=1}^n \bracket[\Bigg]{ 4 \cdot \Exp[\Big]{\poi(\zv)^2 Q_i}
+ \sum_{j \neq i} 4 \cdot \Exp[\Big]{\poi(\zv) \poj(\zv) R_{i,j}}
}
    &\text{(linearity of $\mathbb{E}$)} \\
&= \frac{1}{n^2} \sum_{i=1}^n \bracket[\Big]{ \Var{\dhtesti}
+ \sum_{j \neq i} \Cov{\dhtesti, \dhtestj}
}
    &\text{(Lemmas~\ref{lem:variance-terms} and \ref{lem:covariance-terms})} \\
&= \Var{\dhtest}
\enspace.
\end{align*}
\end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:conservative-variance-estimate}]
% The variance of the \doseht estimator may be expressed in terms of the individual treatment effect estimators as
% \[
% \Var{\dhtest}
% = \Var[\Big]{\frac{1}{n} \sum_{i=1}^n \dhtesti }
% = \frac{1}{n^2} \sum_{i=1}^n \bracket[\Big]{ \Var{\dhtesti} + \sum_{j \neq i} \Cov{\dhtesti, \dhtestj} } 
% \enspace.
% \]
% Because $\Var{\dosei}$, $\Var{\dosej}$, and $\Var{\dosei \dosej}$ are positive for all pairs of outcome units $i,j \in \outunits$, we may apply Lemma~\ref{lem:covariance-terms}.
% By doing so, we obtain that $\Cov{\dhtesti, \dhtestj} = \Exp{\poi(\zv) \poj(\zv) R_{i,j}(\dosei, \dosej)}$ for all pairs of outcome units.
% We may bound the individual variance terms by 
% \[
% \Var{\dhtesti}
% = \Exp{\dhtesti^2} - \Exp{\dhtesti}^2
% \leq \Exp{\dhtesti^2}
% = \Exp[\Big]{\poi(\zv)^2 \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}} }^2 }
% \enspace.
% \]
% Using these together with the linearity of expectation, we have that
% \[
% \Var{\dhtest} 
% \leq \frac{1}{n^2} \sum_{i=1}^n \bracket[\Bigg]{ \Exp[\Big]{\poi(\zv)^2 \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}} }^2} + \sum_{j \neq i} \Exp{\poi(\zv) \poj(\zv) R_{i,j}(\dosei, \dosej)} }
% = \Exp{\erlvarest} \enspace.
% \]
% \end{proof}

% \subsection{Asymptotically Valid Confidence Intervals (Corollary~\ref{cor:confidence-intervals})}

% \ccomment{This is to be written}

==> old-tex/local-search-algorithm.tex <==
\section{Local search algorithm}\label{sec:local-search-alg-appendix}

\begin{algorithm}[H]
\SetAlgoLined
\KwData{$\mathbf W$, the bipartite weight matrix relating diversion units to outcome units}
\KwData{$\phi$, TODO(charshaw)}
\KwData{$R$, the number of local search rounds (suggested value: $200$)}
\KwData{$w_{\max}$, the hard maximum cluster weight}
\KwData{$w_{\min}$, the soft minimum cluster weight (suggested value: $w_{\max}/10$)}
\KwData{$a$, the initial treatment variance penalty (suggested value: $10^4$)}
\KwData{$b$, the penalty decay (suggested value: $0.95$)}
\KwResult{a clustering of the diversion units}
initialize the tables needed for wedge sampling $\mathbf W \mathbf W^T$\;
initialize a clustering where each diversion unit belongs to its own cluster\;
\For{$r = 0$ \KwTo $R - 1$}{
choose a uniform random permutation $\pi$ on diversion units\;
\ForEach{$i \in \pi$} {
choose $j$ with probability proportional to $(\mathbf W \mathbf W^T)_{i, j}$\;
\If{$i$ and $j$ are in different clusters, and moving $i$ to $j$'s cluster won't result in a cluster that weighs more than $w_{\max}$,
and this move improves the objective minus the sum of the squared cluster weights times $a b^r$}{
move $i$ to $j$'s cluster
}
}
}
apply the first-fit decreasing bin packing algorithm with bins of capacity $w_{\min}$ to merge clusters that weigh less than $w_{\min}$
\end{algorithm}

==> old-tex/var-term-est.tex <==

\subsection{Does Lemma 1 work for variances?}

Let's check if Lemma 1 works also to estimate $\Var{\dhtesti}$.
First, recall the lemma.

\begin{manuallemma}{1}
\covariancetermlemma
\end{manuallemma}

Also recall the definition of $R_{i,j}(\dosei, \dosej)$:
\[
R_{i,j}(\dosei, \dosej) =
\frac{ (\dosei - \Exp{\dosei}) (\dosej - \Exp{\dosej})  }{\Var{\dosei} \Var{\dosej} }
- \frac{a \paren{\dosei \dosej - \Exp{\dosei \dosej}} + b \paren{\dosei - \Exp{\dosei}} + c \paren{\dosej - \Exp{\dosej}} }{\beta}.
\]
where
\begin{align*}
a & = \Var{\dosei} \Var{\dosej} + \Cov{\dosei,\dosej}^2 \\
b & = \Var{\dosej} \Cov{\dosei \dosej, \dosei} - \Cov{\dosei,\dosej} \Cov{ \dosei \dosej, \dosej}\\
c & = \Var{\dosei} \Cov{\dosei \dosej, \dosej} - \Cov{\dosei,\dosej} \Cov{ \dosei \dosej, \dosei}\\
\beta &= \Var{\dosei \dosej} \paren{ \Var{\dosei}\Var{\dosej} + \Cov{\dosei, \dosej}^2} \\
    &\quad + \Var{\dosej} \Cov{\dosei \dosej, \dosej}^2 + \Var{\dosei} \Cov{\dosei \dosej, \dosei}^2
    - 2 \Cov{\dosei, \dosej} \Cov{\dosei \dosej,\dosej} \Cov{\dosei \dosej, \dosei}  \enspace.
\end{align*}

At least at first glance, it should be possible to estimate $\Var{\dhtesti}$ unbiasedly with this approach.
In particular, if we set $i = j$, the conditions for Lemma 1 stipulate that $\Var{\dosei} > 0$ and $\Var{\dosei^2} > 0$.
This will be satisfied when $\dosei$ is a random variable in $[-1, 1]$.
Note, however, that this does not hold for binary treatments, $\dosei \in \{-1, 1\}$, because then $\dosei^2 = 1$ with probability one, so $\Var{\dosei^2} = 0$.

When we set $i = j$, we get
\begin{align*}
	\Cov{\dhtesti, \dhtestj} &= \Var{\dhtesti}
	\\
	\Exp{ \poi(\zv) \poj(\zv) R_{i,j}(\dosei, \dosej) } &= \Exp[\Big]{ \bracket{\poi(\zv)}^2 R_{i}(\dosei) }
	\\
	R_{i}(\dosei) &=
		\frac{ (\dosei - \Exp{\dosei})^2  }{\Var{\dosei}^2 }
		- \frac{a \paren{\dosei^2 - \Exp{\dosei^2}} + (b + c) \cdot \paren{\dosei - \Exp{\dosei}}}{\beta}
\end{align*}
with $a = 2 \Var{\dosei}^2$, $b = c = 0$ and $\beta = 2 \Var{\dosei^2} \Var{\dosei}^2$.
Nothing weird so far.

Let's make the proof in reverse order compared to before.
Simialar to before, define
\[
S_{i}(\dosei)
= \frac{ (\dosei - \Exp{\dosei})^2  }{\Var{\dosei}^2 } - R_{i}(\dosei)
= \frac{\dosei^2 - \Exp{\dosei^2}}{\Var{\dosei^2}}.
\]
Consider the definition of the variance:
\begin{equation*}
	\Var{\dhtesti}
	= \Exp{\dhtesti^2} - \Exp{\dhtesti}^2
	= 4 \cdot \Exp[\bigg]{ \bracket{\poi(\zv)}^2  \frac{ (\dosei - \Exp{\dosei})^2  }{\Var{\dosei}^2 }} - 4 m_i^2.
\end{equation*}
Assume for the moment that $\Exp{\dosei^2 S_{i}(\dosei)} = 1$, $\Exp{S_{i}(\dosei) } = 0$ and $\Exp{ \dosei S_{i}(\dosei) } = 0$, then
\begin{align*}
	\Exp[\Big]{ \bracket{\poi(\zv)}^2 S_{i}(\dosei) }
&= \Exp{ (m_i \dosei + b_i)^2 S_{i}(\dosei) } \\
&= m_i^2 \Exp{\dosei^2 S_{i}(\dosei)} + b_i^2 \Exp{S_{i}(\dosei) } + 2 m_i b_i \Exp{ \dosei S_{i}(\dosei) } \\
&= m_i^2,
\end{align*}
which would imply that
\begin{equation*}
	\Var{\dhtesti}
	= 4 \Exp[\Big]{ \bracket{\poi(\zv)}^2 R_{i}(\dosei) }.
\end{equation*}

Let's check whether $S_{i}(\dosei)$ satisfies these conditions.
Two of them are straightforward:
\begin{align*}
	\Exp{\dosei^2 S_{i}(\dosei)} &= \Exp[\bigg]{ \frac{(\dosei^2)^2 - \dosei^2\Exp{\dosei^2}}{\Var{\dosei^2}} } = \frac{\Var{\dosei^2}}{\Var{\dosei^2}} = 1
	\\
	\Exp{S_{i}(\dosei) } &= \Exp[\bigg]{ \frac{\dosei^2 - \Exp{\dosei^2}}{\Var{\dosei^2}} } = 0
\end{align*}
Consider the third term.
We can ignore the denominator, so
\begin{equation*}
	\Exp{\dosei S_{i}(\dosei)} \propto \Exp{\dosei^3} - \Exp{\dosei} \Exp{\dosei^2}.
\end{equation*}
This will not generally be zero.
For example, if the CDF of $\dosei$ is $\Pr(\dosei \leq a) = (a + 1)^2 / 4$, then
\begin{equation*}
	\Exp{\dosei} = \Exp{\dosei^2} = 1/3,
	\qquad\text{and}\qquad
	\Exp{\dosei^3} = 1/5,
\end{equation*}
so $\Exp{\dosei^3} - \Exp{\dosei} \Exp{\dosei^2} = 1/5 - 1/9 = 4 / 45$.

However, an interesting special case is when $\dosei$ is symmetric around zero, so that $\Pr(\dosei = a)$ is equal to $\Pr(\dosei = -a)$ for all $a \in [0, 1]$.
In this case, $\dosei^2$ provides no information about the sign of $\dosei$, which means that
\begin{equation*}
	\Exp{\dosei^3 \mid \dosei^2 = a} = a^{3/2} / 2 - a^{3/2} / 2 = 0.
\end{equation*}
Using the law of total expectation, we have
\begin{equation*}
	\Exp{\dosei^3} = \Exp{\Exp{\dosei^3 \mid \dosei^2}} = 0,
\end{equation*}
and symmetry also gives $\Exp{\dosei} = 0$.
Hence, $\Exp{\dosei S_{i}(\dosei)} = 0$ \emph{if $\dosei$ is symmetric around zero}.
There might be other ways to achieve the same result, but it will not hold in general under the current conditions.


==> tex/proofs.tex <==
\section{Proofs}\label{sec:proofs-appendix}

In this section, we present proofs of the theorems and corollaries in the main paper.
Before continuing, we introduce some notation used in the proofs.
We begin by defining for each outcome unit $i \in \outunits$, an estimate of the individual treatment effect $\itei$, which is
\[
\dhtesti \triangleq 2 \poi(\zv) \paren[\Big]{ \frac{ \dosei(\zv) - \Exp{\dosei(\zv)}}{\Var{\dosei(\zv)}} } \enspace.
\]
Observe that the \doseht estimator is the average of these estimates of the individual treatment effects, i.e. $\dhtest = (1/n) \sum_{i=1}^n \dhtesti$.
Throughout the proofs, we will often reason about the behavior of the \doseht estimator through the properties of the individual treatment effect estimates.

Next, we introduce the statistical concept of \emph{dependency neighborhoods}. 
Let $\erre{1}, \erre{2}, \dots \erre{n}$ be random variables indexed by the integers $[n]$.
For each variable index $i \in [n]$, we define the \emph{dependency neighborhood} as
\[
\depNi = \setb{ j \in [n] : \erri \text{ and } \errj \text{ are not independent}} \enspace.
\]
We take the convention that $i \in \depNi$ and so that each dependency neighborhood as cardinality at least 1.
A measure of dependence between the random variables is the \emph{maximum dependency degree}, which is $\depdeg = \max_{i \in [n]} \abs{\depNi}$.
Note that independent random variables satisfy $D = 1$ and that completely dependent random variables have $D =n$.

For the remainder of the proof, we focus our discussion of dependency neighborhoods and degrees to the collection of errors of the individual treatment effects, 
\[
\erre{1} = \itee{1} - \dhteste{1}, \erre{2} = \itee{2} - \dhteste{2}, \dots \erre{n} = \itee{n} - \dhteste{n} \enspace. 
\]
We begin by showing that in this case, the maximum dependency degree may be bounded in terms of the degrees of the bipartite graph and the dependence in the treatment assignments.

\begin{lemma}\label{lem:dependence-degree-bound}
The dependency degree of the individual treatment effect errors is bounded by $\depdeg \leq \maxcorr \divdeg \outdeg$ .
\end{lemma}
\begin{proof}
First, we establish necessary conditions under which a (random) estimate error $\errj$ is in the dependency neighborhood of the estimate error $\erri$; that is, $j \in \depNi$.
Fix outcome units $i,j \in \outunits$ and consider the estimate errors $\erri = \itei - \dhtesti$ and $\errj = \itej - \dhtestj$.
By the linear exposure assumption, these estimate errors are functions of the random doses $\dosei$ and $\dosej$. 
By the linear dose assumption, these doses, $\dosei$ and $\dosej$, are functions of the random assignments $\zl$ for $\ell \in \divunits$ and $\zve{\ell'}$ for $\ell' \in \neigh(j)$, respectively.
Thus, if $\zl$ and $\zve{\ell'}$ are independent for all pairs $ell \in \neigh(i)$ and $\ell' \in \neigh(j)$, then the doses $\dosei$ and $\dosej$ are independent and so that estimate errors $\erri$ and $\errj$ are independent.
Thus, $j \in \depNi$ only if there exists a pair of assignments $\zl \in \neigh(i)$ and $\zve{\ell'} \in \neigh(j)$ which are dependent.

The remainder of the proof is a counting argument which uses this necessary condition to establish that $\abs{\depNi} \leq \maxcorr \divdeg \outdeg$.
This counting argument is summarized in Figure~XYZ.
Fix an outcome unit $i \in \outunits$ and consider one of the diversion units $\ell \in \neigh(i)$.
By definition of the maximum outcome degree, there are at most $\outdeg$ such diversion units.
This diversion unit $\ell$ has positive weights to at most $\divdeg - 1$ other outcome units, by definition of the maximum diversion degree.
Clearly, the at most $\divdeg - 1$ other outcome units are in $\neigh(i)$.
Additionally, the assignment $\zl$ associated with this diversion unit is dependent with at most $\maxcorr - 1$ other treatment assignments.
The corresponding (at most) $\maxcorr -1$ diversion units are incident to at most $\divdeg$ outcome units, which may also be in $\divNi$.
IN this way, the diversion unit $\ell$ incident to outcome unit $i$ has yielded at most $(\divdeg - 1) + (\maxcorr -1 ) \divdeg = \maxcorr \divdeg - 1$ outcome units which may be in the dependency neighborhood $\depNi$.
Summing over all of the (at most) $\outdeg$ diversion units incident to outcome unit $i$ (and including $i$ itself) yields
\[
\abs{\depNi} \leq (\maxcorr \divdeg - 1) \outdeg + 1
= \maxcorr \divdeg \outdeg - (\outdeg - 1)
\leq \maxcorr \divdeg \outdeg
\]
Taking the maximum of $\abs{\depNi}$ over all $i \in \outunits$ completes the proof, $D = \max_{i \in \outunits} \abs{\depNi} \leq \maxcorr \divdeg \outdeg$.
\end{proof}

\begin{lemma}\label{lem:dose-variance-lower-bound}
If each pair of treatment assignments is non-negatively correlated, then each dose variance is lower bounded as $\Var{\dosei} \geq \frac{4 p (1-p)}{\outdeg}$.
\end{lemma}
\begin{proof}
We begin by expanding the variance of the dose $\dosei$ by
\begin{align*}
\Var{\dosei}
&= \Var{\sum_{j=1}^m w_{i,j} \zj}
    &\text{(definition of dose)} \\
&= \sum_{i=1}^m \bracket[\Big]{ \Var{w_{i,j} \zj} + \sum_{\ell \neq j} \Cov{ w_{i,j} \zj, w_{i,\ell} \zl} }
    &\text{(properties of variance)} \\
&= \sum_{i=1}^m \bracket[\Big]{ w_{i,j}^2 \Var{\zj} + \sum_{\ell \neq j} w_{i,j} w_{i,\ell} \Cov{\zj,\zl} } 
    &\text{(properties of variance and covariance)} \\
&\geq \sum_{i=1}^m w_{i,j}^2 \Var{\zj} 
    &\text{(non-negative weights and correlations)}\\
&= 4 p (1-p) \sum_{i=1}^m w_{i,j}^2 \enspace,
\end{align*}
where the inequality follows because the weights $w_{i,j}$ are non-negative and the assignments are non-negatively correlated and the last equality follows because $\zi$ are $\pm 1$ random variables with $\Pr(\zi = 1) = p$.

We complete the proof by lower bounding the sum of the squares of the weights.
Recall that the sum of the weights is $1$ and there are at most $\outdeg$ non-negative terms in the sum.
Using this together with the inequality that relates $\ell_2$ to $\ell_1$ norms in $d$-dimensions, $\norm{\cdot}_2^2 \geq \frac{1}{d} \norm{\cdot}_1^2$, we have that
\[
\sum_{i=1}^m w_{i,j}^2 
\geq \frac{1}{\outdeg} \sum_{i=1}^m w_{i,j}
= \frac{1}{\outdeg} \enspace. \qedhere
\]
\end{proof}

\begin{lemma}\label{lem:ite-error-moments}
The $p$th moment of the error of the individual treatment effect estimates is bounded by
\[
\Exp{ \abs{\itei - \dhtesti}^p }
\leq \bracket[\Bigg]{2 \maxpo \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}}}^p \enspace.
\]
\end{lemma}
\begin{proof}
We begin by remarking that $\abs{\poi(\zv)} \leq M$ implies that each of the individual slopes are also bounded in absolute value as $\abs{m_i} \leq M$.
Recall that by the linear response assumption, $\poi(\zv) = m_i \dosei + b_i$ and by the linear dose assumption (along with the normalization of the edge weights), setting $\zv = \pm \onevec$ results in a dose of $\xi = \pm 1$.
Thus, when considering $\zv = \pm 1 \onevec$, the bound $\abs{\poi(\zv)} \leq M$ implies that $\abs{\pm m_i + b_i} \leq M$, which is enough to establish that $\abs{m_i} \leq M$.
We provide a quick sketch here: suppose that $b_i$ is positive.
In this case, $\abs{m_i + b_i} \leq M$ implies $m_i + b_i \leq M$, which further implies that $m_i \leq M - b_i \leq M$.
Likewise, $\abs{m_i + b_i} \leq M$ implies $-m_i - b_i \geq -M$, which further implies that $-m_i \geq -M + b_i \geq M$.
This establishes that $\abs{m_i} \leq M$ when $b_i$ is positive and the non-positive case follows in a similar fashion.

We now proceed by proving a bound on $\abs{\itei - \dhtesti}$, which holds for any realization of the random variables:
\begin{align*}
\abs{\itei - \dhtesti}
&= \abs[\Big]{2 m_i - 2 \poi(\zv) \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} } \\
&\leq 2 \abs{m_i} + 2 \frac{\abs{\poi(\zv)} \cdot \abs{\dosei - \Exp{\dosei}}}{\Var{\dosei}} 
    &\text{(triangle inequality)}\\
&\leq 2 \maxpo + 2 \frac{\maxpo \cdot 2}{\Var{\dosei}} 
    &\text{(definition of $\maxpo$ and above)}\\
&\leq 2 \maxpo \paren[\Big]{ 1 + \frac{2}{\Var{\dosei}} } 
    &\text{(collecting terms)}\\
&\leq 2 \maxpo \paren[\Big]{1 + \frac{\outdeg}{2 p(1-p)}}
    &\text{(Lemma~\ref{lem:dose-variance-lower-bound})}
\end{align*}
The moment bound follows by applying the bound above.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:consistency} (Consistent)}

\begin{manualtheorem}{\ref{thm:consistency}}
\consistencythm
\end{manualtheorem}
\begin{proof}
We begin by proving a finite sample bound on the mean squared error of the \doseht estimator, and then we finish the proof by taking the limit in the asymptotic sequence.
Note that the mean squared error may be broken down into the errors of the individual treatment effect estimates via
\[
\Exp{(\ate - \dhtest)^2}
= \Exp[\Big]{\paren[\Big]{ \frac{1}{n} \sum_{i=1}^n \itei - \dhtesti }^2 }
= \frac{1}{n^2} \sum_{i=1}^n \paren[\Bigg]{ \Exp{ (\itei - \dhtesti)^2 } + \sum_{j \neq i} \Exp{(\itei - \dhtesti)(\itej - \dhtestj)} } 
\enspace.
\]
Note that the term in the inner sum is the covariance of the errors in the individual treatment effect estimates.
By definition of the dependency neighborhoods, only terms $j \in \depNi$ are dependent and so only these terms will have non-zero covariance.
Using this and the second moment bound in Lemma~\ref{lem:ite-error-moments}, we have that
\begin{align*}
\Exp{(\ate - \dhtest)^2}
&= \frac{1}{n^2} \sum_{i=1}^n \paren[\Bigg]{ \Exp{ (\itei - \dhtesti)^2 } + \sum_{\substack{j \in \depNi \\ j \neq i}} \Exp{(\itei - \dhtesti)(\itej - \dhtestj)} } 
    &\text{(dependency neighborhoods)} \\
&\leq \frac{1}{n^2} \sum_{i=1}^n \paren[\Bigg]{ \Exp{ (\itei - \dhtesti)^2 } + \sum_{\substack{j \in \depNi \\ j \neq i}} \sqrt{ \Exp{(\itei - \dhtesti)^2} \Exp{(\itej - \dhtestj)^2}} } 
    &\text{(Cauchy-Schwarz)} \\
&\leq \frac{1}{n^2} \sum_{i=1}^n \abs{\depNi} \cdot \bracket[\Big]{2 M \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}} }^2
    &\text{(Lemma~\ref{lem:ite-error-moments})} \\
&\leq \frac{\depdeg}{n} \bracket[\Big]{2 M \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}} }^2 \enspace.
    &\text{(max dependency degree)}
\end{align*}
By using the bound $\depdeg \leq \maxcorr \divdeg \outdeg$ given in Lemma~\ref{lem:dependence-degree-bound}, we have the finite-sample bound on the mean squared error:
\[
\Exp{(\ate - \dhtest)^2}
\leq \frac{\maxcorr \divdeg \outdeg  }{n} \bracket[\Big]{2 M \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}} }^2
\]

We now interpret this finite-sample bound in the context of the asymptotic sequence.
By Assumptions~XYZ, we have that $M$ is a constant and $p$ is bounded away from $0$ and $1$ by a constant.
It follows that the mean squared error is asymptotically bounded by the rate $\Exp{(\ate - \dhtest)^2} = \bigO{\maxcorr \divdeg \outdeg^3 / n}$.
By assumption, the asymptotic sequence satisfies $\maxcorr \divdeg \outdeg^3 = \littleO{n}$, and thus the mean squared error converges to zero under these conditions.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:asymptotic-normality} (Asymptotic Normality)}

\begin{lemma}[Lemma 3.6 of \cite{ross2011fundamentals}] \label{lem:steins-method}
Let $\erre{1}, \erre{2}, \dots \erre{n}$ be random variables such that $\Exp{\erri^4} < \infty$, $\Exp{\erri} = 0$, $\sigma^2 = \Var{\frac{1}{n} \sum_{i=1}^n \erri}$, and define $X = \paren{\frac{1}{n} \sum_{i=1}^n \erri} / \sigma$.
Then for a standard normal $Z \sim \mathcal{N}(0,1)$, we have
\[
d_W(X,Z) \leq 
\frac{D^2}{\sigma^3 n^3} \sum_{i=1}^n \Exp{\abs{\erri}^3} 
+ \sqrt{\frac{28}{\pi}} \cdot \frac{\depdeg^{3/2}}{n^2 \sigma^2} \sqrt{ \sum_{i=1}^n \Exp{\erri^4} }
\enspace,
\]
where $\depdeg$ is the maximum dependency degree of the random variables and $d_W(\cdot, \cdot)$ is the Wasserstein distance.
\end{lemma}

\begin{manualtheorem}{\ref{thm:asymptotic-normality}}
\asymptoticanormalitythm
\end{manualtheorem}
\begin{proof}
Our strategy may be described in two main steps: first, we use Lemma~\ref{lem:steins-method} to derive a finite-sample bound on the Wasserstein distance between the distribution of $(\ate - \dhtest) / \sqrt{\Var{\dhtest}}$ and a standard normal. Next, we us this bound to argue that this Wasserstein distance approaches $0$ in the limit of the asymptotic sequence under the above conditions.

We seek to apply Lemma~\ref{lem:steins-method} where the random variables are the errors of the individual treatment effect estimates; that is,
\[
\erre{1} = \itee{1} - \dhteste{1}, \erre{2} = \itee{2} - \dhteste{2}, \dots \erre{n} = \itee{n} - \dhteste{n} \enspace. 
\]
Note that $\frac{1}{n} \sum_{i=1}^n \erri = \frac{1}{n} \sum_{i=1}^n \itei - \dhtesti = \ate - \dhtest$ and $\Var{\frac{1}{n} \sum_{i=1}^n \erri} = \Var{\dhtest}$ so that the random variable $X$ in Lemma~\ref{lem:steins-method} is equal to $(\ate - \dhtest) / \sqrt{\Var{\dhtest}}$, which is the random variable we which to characterize.
Let's show that the conditions of Lemma~\ref{lem:steins-method} are satisfied: first, recall that $\dhtesti$ are unbiased estimates of $\itei$ so that $\erri$ has mean zero.
Second, because the potential outcomes are bounded by a constant $\maxpo$, the support of $\erri$ is bounded so the fourth moments are finite.
Thus, we may apply Lemma~\ref{lem:steins-method} in this setting.

We will use the Lemma~\ref{lem:ite-error-moments} to bound the sum of the third and fourth moments.
In particular, Lemma~\ref{lem:ite-error-moments} implies that
\[
\sum_{i=1}^n \Exp{\abs{\erri}^3} \leq n \cdot \bracket[\Bigg]{2 \maxpo \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}}}^3 
\quad \text{ and } \quad
\sum_{i=1}^n \Exp{\abs{\erri}^4} \leq n \cdot \bracket[\Bigg]{2 \maxpo \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}}}^4
\enspace.
\]
Using this moment bound together with the bound on the maximum dependence degree $\depdeg$ (Lemma~\ref{lem:dependence-degree-bound}) on the result of Lemma~\ref{lem:steins-method}, we obtain that
\[
d_W\paren[\Big]{\frac{\ate - \dhtest}{\sqrt{\Var{\dhtest}}}, Z} \leq
\frac{(\maxcorr \divdeg \outdeg)^2}{\sigma^3 n^2} \cdot \bracket[\Bigg]{2 \maxpo \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}}}^3 
+
\sqrt{\frac{28}{\pi}} \cdot
\frac{(\maxcorr \divdeg \outdeg)^{3/2}}{\sigma^2 n^{3/2}} \cdot \bracket[\Bigg]{2 \maxpo \paren[\Big]{1 + \frac{\outdeg}{2p(1-p)}}}^2
\]

We now interpret this finite-sample bound in the context of the asymptotic sequence.
By Assumptions~XYZ, we have that $M$ is a constant and $p$ is bounded away from $0$ and $1$ by a constant.
It follows that the Wasserstein distance between $(\ate - \dhtest) / \sqrt{\Var{\dhtest}}$ and a standard normal is asymptotically bounded by
\[
d_W\paren[\Big]{\frac{\ate - \dhtest}{\sqrt{\Var{\dhtest}}}, Z}
= \bigO[\Big]{
\frac{(\maxcorr \divdeg)^2 \outdeg^5}{\sigma^3 n^2}
+ \frac{(\maxcorr \divdeg)^{3/2} \outdeg^{3.5}}{\sigma^2 n^{3/2}}
}
\]
By Assumption~XYZ, we have that $\Var{\dhtest} = \bigOmega{n^{-1/2}}$, which means that this bound becomes
\[
d_W\paren[\Big]{\frac{\ate - \dhtest}{\sqrt{\Var{\dhtest}}}, Z}
= \bigO[\Big]{
\frac{(\maxcorr \divdeg)^2 \outdeg^5}{n^{5/4}}
+ \frac{(\maxcorr \divdeg)^{3/2} \outdeg^{3.5}}{n} \enspace.
}
\]
By assumption, the asymptotic sequence satisfies $(\maxcorr \divdeg)^2 \outdeg^5 = \littleO{n^{5/4}}$ and $(\maxcorr \divdeg)^{3/2} \outdeg^{3.5} = \littleO{n}$.
Thus, the Wasserstein distance between $(\ate - \dhtest) / \sqrt{\Var{\dhtest}}$ and a standard normal approaches $0$ in this asymptotic sequence.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:conservative-variance-estimate} (Conservative Variance Estimate)}

\begin{manualtheorem}{\ref{thm:conservative-variance-estimate}}
\conservativevarest
\end{manualtheorem}

For each pair of outcome units $i,j \in \outunits$, define the function $S_{i,j}(\dosei, \dosej)$ to be the second term in the function $R_{i,j}(\dosei, \dosej)$; that is,
\[
S_{i,j}(\dosei, \dosej) =
\frac{a \paren{\dosei \dosej - \Exp{\dosei \dosej}} + b \paren{\dosei - \Exp{\dosei}} + c \paren{\dosej - \Exp{\dosej}} }{\beta} \enspace,
\]
where $a,b,c,\beta$ are defined as 
\begin{align*}
    a & = \Var{\dosei} \Var{\dosej} + \Cov{\dosei,\dosej}^2 \\
    b & = \Var{\dosej} \Cov{\dosei \dosej, \dosei} - \Cov{\dosei,\dosej} \Cov{ \dosei \dosej, \dosej}\\
    c & = \Var{\dosei} \Cov{\dosei \dosej, \dosej} - \Cov{\dosei,\dosej} \Cov{ \dosei \dosej, \dosei}\\
\end{align*}
and the normalization term in the denominator is given by 
\begin{align*}
  \beta 
&= \Var{\dosei \dosej} \paren{ \Var{\dosei}\Var{\dosej} + \Cov{\dosei, \dosej}^2} \\
&\quad + \Var{\dosej} \Cov{\dosei \dosej, \dosej}^2 + \Var{\dosei} \Cov{\dosei \dosej, \dosei}^2 
- 2 \Cov{\dosei, \dosej} \Cov{\dosei \dosej,\dosej} \Cov{\dosei \dosej, \dosei}  
\enspace.
\end{align*}
In this way, $R_{i,j}(\dosei,\dosej) \triangleq \paren{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} + S_{i,j}(\dosei, \dosej)$.

\begin{lemma}\label{lem:properties-of-S}
Fix a pair of outcome units $i,j \in \outunits$. 
If $\Var{\dosei}$, $\Var{\dosej}$, and $\Var{\dosei \dosej}$ are positive then the function $S_{i,j}(\dosei, \dosej)$ satisfies the following properties:
\begin{itemize}
    \item $\Exp{S_{i,j}(\dosei, \dosej)} = 0$
    \item $\Exp{\dosei S_{i,j}(\dosei, \dosej)} = \Exp{\dosej S_{i,j}(\dosei, \dosej)} = 0$
    \item $\Exp{\dosei \dosej S_{i,j}(\dosei, \dosej)} = 1$
\end{itemize}
\end{lemma}
\begin{proof}
For notational simplicity, we will drop the subscripts and write $\dosei$ as $x$, $\dosej$ as $y$ and $S_{i,j}(\dosei, \dosej)$ as $S(x,y)$.

First, let's verify that the normalization term $\beta$ is positive when $\Var{\dosei}$, $\Var{\dosej}$, and $\Var{\dosei \dosej}$ are also positive.
Recall that the normalization term $\beta$ is defined as
\begin{align*}
  \beta 
&= \Var{xy} \left( \Var{x}\Var{y} + \Cov{x,y}^2 \right) \\
&+ \Var{y} \Cov{xy,x}^2 + \Var{x} \Cov{xy,y}^2  - 2 \Cov{x,y} \Cov{xy,y} \Cov{xy,x}  
\end{align*}
Denote $\sigma_x = \sqrt{\Var{x}}$ and $\sigma_y = \sqrt{\Var{y}}$.
and let $s \in \{ \pm 1 \}$ be given.
By completing the square, we may write the terms
\[
\Var{y} \Cov{xy,x}^2 + \Var{x} \Cov{xy,y}^2 
= ( \sigma_y \Cov{xy,x} + s \sigma_x \Cov{xy,y} )^2 - 2 s \sigma_x \sigma_y \Cov{xy,x} \Cov{xy,y}
\]
and substituting this into the definition of $\beta$ yields
\begin{align*}
  \beta 
&= \Var{xy} \left( \Var{x}\Var{y} + \Cov{x,y}^2 \right) \\
&\quad + ( \sigma_y \Cov{xy,x} + s \sigma_x \Cov{xy,y} )^2 
- 2(s \sigma_x \sigma_y - \Cov{x,y}) \Cov{xy,y} \Cov{xy,x} \\
&= \Var{xy} \left( \Var{x}\Var{y} + \Cov{x,y}^2 \right) \\
&\quad + ( \sigma_y \Cov{xy,x} + s \sigma_x \Cov{xy,y} )^2
- 2s (\sigma_x \sigma_y - s \Cov{x,y}) \Cov{xy,y} \Cov{xy,x} \enspace,
\end{align*}
Note that the first two terms are non-negative.
We will now show that for an appropriate choice of $s \in \{ \pm 1 \}$, the third term is also non-negative.
By the Cauchy-Schwarz inequality, $| \Cov{x,y} | \leq \sigma_x \sigma_y$ so that the factor $(\sigma_x \sigma_y - s \Cov{x,y})$ in the third term is non-negative.
Thus, by setting $s = - \textrm{sign}\left( \Cov{xy,y} \Cov{xy,x} \right) $, the third term is non-negative.
This establishes that the normalization term $\beta$ is non-negative.
The condition $\Var{x}, \Var{y}, \Var{xy} > 0$ ensures that the first term is positive so that $\beta$ is positive.

Next, we verify the three properties in the lemma.
The first is easy to verify by the linearity of expectation, as
\[
\beta \cdot \Exp{S(x,y)} 
= \Exp{ a(xy - \Exp{xy}) + b (x - \Exp{x}) + c (y - \Exp{y}) }
= 0 
\]
so that dividing both sides by $\beta$ yields the desired result.

We now verify the second property.
Observe that
\begin{align*}
\beta \cdot \Exp{x S(x,y)} 
&= a \cdot ( \Exp{x^2 y} - \Exp{x}\Exp{xy}) + b \cdot (\Exp{x^2} - \Exp{x}^2) + c \cdot (\Exp{xy} - \Exp{x}\Exp{y}) \\
&= a \cdot \Cov{xy,x} + b \cdot \Var{x} + c \cdot \Cov{x,y} \\
&= \Cov{xy,x} (\Var{x} \Var{y} + \Cov{x,y}^2) \\
&\quad\quad+ \Var{x} (\Var{y} \Cov{xy,x} - \Cov{x,y} \Cov{xy,y}) \\
&\quad\quad + \Cov{x,y}(\Var{x} \Cov{xy,y} - \Cov{x,y} \Cov{xy,x}) \\
&= 0 \enspace,
\end{align*}
and dividing both sides by $\beta$ yields the desired result.
The proof that $\Exp{y S(x,y)} = 0$ follows in exactly the same fashion.

Finally, we verify the third property.
Observe that
\begin{align*}
\beta \cdot \Exp{x S(x,y)} 
&= a \cdot ( \Exp{(xy)^2} - \Exp{xy}^2) + b \cdot (\Exp{x^2y} - \Exp{xy} \Exp{x}) + c \cdot (\Exp{xy^2} - \Exp{xy} \Exp{y}) \\
&= a \cdot \Var{xy} + b \cdot \Cov{xy,x} + c \cdot \Cov{xy,y} \\
&= \Var{xy} (\Var{x} \Var{y} + \Cov{x,y}^2) \\
&\quad\quad+ \Cov{xy,x} (\Var{y} \Cov{xy,x} - \Cov{x,y} \Cov{xy,y}) \\
&\quad\quad + \Cov{xy,y}(\Var{x} \Cov{xy,y} - \Cov{x,y} \Cov{xy,x}) \\
&= \Var{xy} (\Var{x} \Var{y} + \Cov{x,y}^2) \\
&\quad\quad + \Var{y} \Cov{xy,x}^2 + \Var{x} \Cov{xy,y}^2  \\
&\quad\quad - 2 \Cov{x,y} \Cov{xy,y} \Cov{xy,x} \\
&= \beta \enspace,
\end{align*}
so that dividing both sides by $\beta$ yields the desired result.
\end{proof}

\begin{manuallemma}{\ref{lem:covariance-terms}}
\covariancetermlemma
\end{manuallemma}

\begin{proof}
Because the individual treatment effect estimates are unbiased,
\begin{align*}
\Cov{\dhtesti, \dhtestj} 
&= \Exp{\dhtesti \dhtestj} - \Exp{\dhtesti} \Exp{\dhtestj} \\
&= \Exp{\dhtesti \dhtestj} - \itei \itej \\
&= 4 \cdot \Exp[\Big]{\poi(\zv) \poj(\zv) \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} }
- 4 m_i m_j
\end{align*}
Because $\Var{\dosei}$, $\Var{\dosej}$, and $\Var{\dosei \dosej}$ are positive, we may use the properties of the function $S_{i,j}(\dosei, \dosej)$ proved in Lemma~\ref{lem:properties-of-S}.
Using this lemma together with the linear response assumption yields that
\begin{align*}
\Exp{ \poi(\zv) \poj(\zv) S_{i,j}(\dosei, \dosej) }
&= \Exp{ (m_i \dosei + b_i) (m_j \dosej + b_j) S_{i,j}(\dosei, \dosej) } 
    &\text{(linear response)}\\
&= m_i m_j\Exp{\dosei \dosej S_{i,j}(\dosei, \dosej)} + b_i b_j \Exp{S_{i,j}(\dosei, \dosej) } \\
&\quad + m_i b_j \Exp{ \dosei S_{i,j}(\dosei, \dosej) } + m_j b_i \Exp{ \dosej S_{i,j}(\dosei, \dosej) } 
    &\text{(expanding terms)}\\
&= m_i m_j
    \enspace.
    &\text{(Lemma~\ref{lem:properties-of-S})} 
\end{align*}
The proof is completed by recalling that $R_{i,j}(\dosei,\dosej) \triangleq \paren{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} + S_{i,j}(\dosei, \dosej)$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:conservative-variance-estimate}]
The variance of the \doseht estimator may be expressed in terms of the individual treatment effect estimators as
\[
\Var{\dhtest}
= \Var[\Big]{\frac{1}{n} \sum_{i=1}^n \dhtesti }
= \frac{1}{n^2} \sum_{i=1}^n \bracket[\Big]{ \Var{\dhtesti} + \sum_{j \neq i} \Cov{\dhtesti, \dhtestj} } 
\enspace.
\]
Because $\Var{\dosei}$, $\Var{\dosej}$, and $\Var{\dosei \dosej}$ are positive for all pairs of outcome units $i,j \in \outunits$, we may apply Lemma~\ref{lem:covariance-terms}.
By doing so, we obtain that $\Cov{\dhtesti, \dhtestj} = \Exp{\poi(\zv) \poj(\zv) R_{i,j}(\dosei, \dosej)}$ for all pairs of outcome units.
We may bound the individual variance terms by 
\[
\Var{\dhtesti}
= \Exp{\dhtesti^2} - \Exp{\dhtesti}^2
\leq \Exp{\dhtesti^2}
= \Exp[\Big]{\poi(\zv)^2 \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}} }^2 }
\enspace.
\]
Using these together with the linearity of expectation, we have that
\[
\Var{\dhtest} 
\leq \frac{1}{n^2} \sum_{i=1}^n \bracket[\Bigg]{ \Exp[\Big]{\poi(\zv)^2 \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}} }^2} + \sum_{j \neq i} \Exp{\poi(\zv) \poj(\zv) R_{i,j}(\dosei, \dosej)} }
= \Exp{\erlvarest} \enspace.
\]
\end{proof}

\subsection{Proof of Corollary~\ref{cor:confidence-intervals} (Asymptotically Valid Confidence Intervals)}

\subsection{Mean Squared Error}\label{sec:mse-proofs}
In this section, we give the proofs of Propositions~\ref{claim:doseht-variance-no-slope} and \ref{claim:doseht-variance-no-intercept}, which are concerned with the mean squared error of the \doseht estimator.
Along the way, we derive a general form for the mean squared error of the \doseht estimator.

We begin by defining for each outcome unit $i \in \outunits$
\[
\dhtesti \triangleq 2 \poi(\zv) \paren[\Big]{ \frac{ \dosei(\zv) - \Exp{\dosei(\zv)}}{\Var{\dosei(\zv)}} } \enspace,
\]
which is an estimator of the individual treatment effect $\itei$.
Observe that the \doseht estimator is the average of these estimates of the individual treatment effects, i.e. $\dhtest = (1/n) \sum_{i=1}^n \dhtesti$.
In the proof of Theorem~\ref{thm:exposure-ht-unbiased}, we established unbiasedness of $\dhtest$ by establishing unbiasedness of these estimates of the individual treatment effects, i.e. $\Exp{\dhtesti} = \itei$.
In a similar way, we can derive the mean squared error of the \doseht estimator in terms of the variance and covariance of the estimates of individual treatment effects.
We give a general expression for the mean squared error of the \doseht estimator below in Lemma~\ref{lemma:mse-derivation}.

\begin{lemma}\label{lemma:mse-derivation}
Under the linear response assumption, the mean squared error of the \doseht estimator is given by
\[
\Exp{ \paren{ \dhtest - \ate}^2} 
= \frac{1}{n^2} \bracket[\Bigg]{ \sum_{i=1}^n \Var{\dhtesti} + 2 \sum_{i < j} \Cov{\dhtesti, \dhtestj}}
\]
where
\begin{align*}
\Var{\dhtesti} &= 4 
\Exp[\Bigg]{ \paren[\Bigg]{ m_i \paren[\Big]{ \frac{\dosei^2 - \dosei \Exp{\dosei}}{\Var{\dosei}} - 1 } + b_i \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} }^2 } \\
\text{and } \quad \Cov{\dhtesti, \dhtestj} &= 4 
\Exp[\Bigg]{ \paren{m_i \dosei + b_i} \paren{m_j \dosej + b_j} \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}}
} - 4 m_i m_j \enspace.
\end{align*}
\end{lemma}
\begin{proof}
First, recall that $\dhtest = \frac{1}{n} \sum_{i=1}^n \dhtesti$.
Using that $\dhtest$ is an unbiased estimate of $\ate$ and by properties of variance, we have that
\[
\Exp{ \paren{ \dhtest - \ate}^2} 
= \Var{ \dhtest} 
= \Var[\Big]{ \frac{1}{n} \sum_{i=1}^n \dhtesti }
= \frac{1}{n^2} \bracket[\Big]{ \sum_{i=1}^n \Var{\dhtesti} + 2 \sum_{i < j} \Cov{\dhtesti, \dhtestj}}
\]
Using the linear response assumption, the individual variance terms may be obtained as 
\begin{align*}
\Var{\dhtesti}
&= \Exp{\paren{\dhtesti - \itei}^2} \\
&= \Exp[\Bigg]{ \paren[\Bigg]{2 \poi(\dosei) \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} - 2 m_i }^2} \\
&= 4 \Exp[\Bigg]{\paren[\Bigg]{\paren{m_i \dosei + b_i} \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} - m_i }^2} \\
&= 4 \Exp[\Bigg]{ \paren[\Bigg]{ m_i \paren[\Big]{ \frac{\dosei^2 - \dosei \Exp{\dosei}}{\Var{\dosei}} - 1 } + b_i \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} }^2 } \enspace.
\end{align*}

In a similar fashion, the covariance terms may be obtained as
\begin{align*}
\Cov{\dhtesti, \dhtestj}
&= \Exp{\dhtesti \dhtestj} - \Exp{\dhtesti}\Exp{\dhtestj} \\
&= \Exp[\Bigg]{2\poi(\dosei)\paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \cdot 2\poj(\dosej)\paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} } - (2m_i)(2m_j) \\
&= 4 
\Exp[\Bigg]{ \paren{m_i \dosei + b_i} \paren{m_j \dosej + b_j} \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}}
} - 4 m_i m_j
\end{align*}
\end{proof}

Using this general expression for the mean squared error, we can easily prove Propositions~\ref{claim:doseht-variance-no-slope} and \ref{claim:doseht-variance-no-intercept}.
For completeness, we restate the propositions here.

\begin{manualtheorem}{\ref{claim:doseht-variance-no-slope}}
\mseNoSlope
\end{manualtheorem}
\begin{proof} %[Proof of Proposition~\ref{claim:doseht-variance-no-slope}]
Setting $m_i = 0$ yields
\[
\Var{\dhtesti} 
= 4 \Exp[\Bigg]{b_i^2 \frac{\paren{\dosei - \Exp{\dosei}}^2}{\Var{\dosei}^2}}
= 4 b_i^2 \frac{\Var{\dosei}}{\Var{\dosei}^2}
= 4 b_i^2 \frac{1}{\Var{\dosei}}
\]
and
\[
\Cov{\dhtesti, \dhtestj}
= 4 \Exp[\Bigg]{b_i b_j \paren[\Big]{\frac{\dosei - \Exp{\dosei}}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej - \Exp{\dosej}}{\Var{\dosej}}} }
= 4 b_i b_j \frac{\Cov{\dosei, \dosej}}{\Var{\dosei} \Var{\dosej}}
\]
By Lemma~\ref{lemma:mse-derivation}, this yields the mean squared error
\[
\Exp{ \paren{ \dhtest - \ate}^2} 
= \frac{1}{n^2} \bracket[\Bigg]{ \sum_{i=1}^n \Var{\dhtesti} + 2 \sum_{i < j} \Cov{\dhtesti, \dhtestj}}
= \frac{4}{n^2} \bracket[\Bigg]{ \sum_{i=1}^n b_i^2 \frac{1}{\Var{\dosei}} + 2 \sum_{i<j} b_i b_j \frac{\Cov{\dosei, \dosej}}{\Var{\dosei} \Var{\dosej}} } \enspace,
\]
as desired.
\end{proof}

\begin{manualtheorem}{\ref{claim:doseht-variance-no-intercept}}
\mseNoIntercept
\end{manualtheorem}
\begin{proof} %[Proof of Proposition~\ref{claim:doseht-variance-no-intercept}]
If both treatment assignments are equally likely for all diversion units, then $\Exp{\zi} = 0$.
By linearity, this implies that $\Exp{\dosei} = 0$.
Using this and setting $b_i = 0$ yields
\begin{align*}
\Var{\dhtesti} 
&= 4 \Exp[\Bigg]{m_i^2 \paren[\Big]{ \frac{\dosei^2}{\Var{\dosei}} - 1}^2 } \\
&= 4 m_i^2 \paren[\Big]{ \frac{\Exp{\dosei^4}}{\Var{\dosei}^2} - 2\frac{\Exp{\dosei^2}}{\Var{\dosei}} + 1} 
    &\text{(linearity of expectation)}\\
&\leq 4 m_i^2 \paren[\Big]{ \frac{\Exp{\dosei^2}}{\Var{\dosei}^2} - 2\frac{\Exp{\dosei^2}}{\Var{\dosei}} + 1} 
&\text{($\dosei^4 \leq \dosei^2$ for $\dosei \in [-1,1]$)}\\
&= 4 m_i^2 \paren[\Big]{ \frac{\Var{\dosei}}{\Var{\dosei}^2} - 2\frac{\Var{\dosei}}{\Var{\dosei}} + 1} 
&\text{($\Exp{\dosei} = 0 \Rightarrow \Exp{\dosei^2} = \Var{\dosei}$)} \\
&= 4 m_i^2 \paren[\Big]{ \frac{1}{\Var{\dosei}} - 1 }
\end{align*}
Likewise, using $\Exp{\dosei} = 0$ and $b_i = 0$ yields
\begin{align*}
\Cov{\dhtesti, \dhtestj}
&= 4 \Exp[\Bigg]{ m_i \dosei m_j \dosej \paren[\Big]{\frac{\dosei}{\Var{\dosei}}} \paren[\Big]{\frac{\dosej}{\Var{\dosej}}} } - 4 m_i m_j \\
&= 4 m_i m_j \frac{\Exp{\dosei^2 \dosej^2}}{\Var{\dosei} \Var{\dosej}} - 4 m_i m_j \\
&= 4 m_i m_j \paren[\Bigg]{\frac{\Exp{\dosei^2 \dosej^2}}{\Var{\dosei} \Var{\dosej}} - 1} \enspace.
\end{align*}
By Lemma~\ref{lemma:mse-derivation}, this yields the upper bound on the mean squared error
\begin{align*}
\Exp{ \paren{ \dhtest - \ate}^2} 
&= \frac{1}{n^2} \bracket[\Bigg]{ \sum_{i=1}^n \Var{\dhtesti} + 2 \sum_{i < j} \Cov{\dhtesti, \dhtestj}} \\
&\leq \frac{4}{n^2} \bracket[\Bigg]{ \sum_{i=1}^n m_i^2 \paren[\Big]{ \frac{1}{\Var{\dosei}} - 1 } + 2 \sum_{i<j} m_i m_j \paren[\Bigg]{\frac{\Exp{\dosei^2 \dosej^2}}{\Var{\dosei} \Var{\dosej}} - 1} } \enspace,
\end{align*}
as desired.
\end{proof}

\subsection{\exposuredesign and Correlation Clustering}\label{sec:corr-cluster-proofs}

In this section, we prove the relationship between \exposuredesign, its reformulation \corrclust, the previously proposed correlation clustering design of \cite{pouget2019variance}, and other correlation clustering variants.
A summary of the results are:
\begin{itemize}
    \item In Section~\ref{sec:reformulation}, we show that the \exposuredesign may be reformulated as the clustering problem, \corrclust.
    \item In Section~\ref{sec:prev_instance}, we compare \exposuredesign to the correlation clustering-based design presented in \cite{pouget2019variance}. In particular, we prove that their design is equivalent to \exposuredesign when the trade-off parameter is set as $\phi = 1/(n-1)$.
    \item In Section~\ref{sec:comparing_variants}, we compare \corrclust to other correlation clustering variants. In particular, we prove that \corrclust may be viewed as an instance of the weighted maximization correlation clustering considered by \cite{CGV05clustering, Swamy04correlation} but with a possibly large additive constant which prevents an approximation-preserving reduction.
\end{itemize}

To begin, we demonstrate how to re-write the \corrclust objective using matrix notation.
Let $\omega_{i,j} \in \Reals$ be the weights for pairs $i,j \in [m]$ and let $\Omega$ be the $m$-by-$m$ matrix whose $(i,j)$th entry is $\omega_{i,j}$.
For a partition $\clustering$ of the indices $[m]$, let $Z_\clustering$ be the $m$-by-$m$ matrix where the $(i,j)$th entry is $1$ if $i$ and $j$ are in the same cluster of $\clustering$ and $0$ otherwise.
Then, we may express the \corrclust objective as
\[
\sum_{\cluste{r} \in \clustering} \sum_{i,j \in \cluste{r}} \omega_{i,j}
=
\sum_{i=1}^n \sum_{j=1}^n \omega_{i,j} \bracket{Z_\clustering}_{(i,j)}
= \tr{ \Omega \ Z_\clustering } \enspace.
\]
Throughout the remainder of the section, it will be useful to write the \corrclust objective using this matrix notation.

\subsubsection{Reformulating \exposuredesign as \corrclust}\label{sec:reformulation}
We are now ready to prove Proposition~\ref{prop:corr_cluster_instance}, which we restate here for completeness.


\begin{manualtheorem}{\ref{prop:corr_cluster_instance}}
\corrClustInstance
\end{manualtheorem}
\begin{proof}
Recall that the objective of \exposuredesign is defined as
\[
\max_{\text{clustering} \clustering} \sum_{i=1}^n \Var{\dosei} - \phi \sum_{i \neq j} \Cov{ \dosei, \dosej} \enspace,
\]
where the expectation in the variance and covariance terms is taken with respect to the random assignment vector $\zv \in \setb{\pm 1}^m$, which is drawn from the cluster design given by $\clustering$.
Recall that the exposures are given by $\dosev = \weightM \zv$.
Using matrix notation, we can more compactly represent this objective as
\begin{align*}
\sum_{i=1}^n \Var{\dosei} - \phi \sum_{i \neq j} \Cov{ \dosei, \dosej}
&= \tr[\Big]{ \paren[\big]{\idM - \phi \paren{\onevec \onevec^\tran - \idM}} \Cov{\dosev} } 
    &\text{(rewriting in terms of $\trm$)}\\
&= \tr[\Big]{ \paren[\big]{\paren{1+\phi}\idM - \phi \onevec \onevec^\tran} \Cov{\dosev} }
    &\text{(rearranging terms)} \\
&= \tr[\Big]{ \paren[\big]{\paren{1+\phi}\idM - \phi \onevec \onevec^\tran} \Cov{\weightM \zv} }
    &\text{(definition of exposure)} \\
&= \tr[\Big]{ \paren[\big]{\paren{1+\phi}\idM - \phi \onevec \onevec^\tran} \weightM \Cov{\zv} \weightM^\tran }
    &\text{(property of covariance)} \\
&= \tr[\Big]{ \weightM^\tran \paren[\big]{\paren{1+\phi}\idM - \phi \onevec \onevec^\tran} \weightM \Cov{\zv}}
    &\text{(cyclic property of trace)} \\
\end{align*}
Because $\zv$ is drawn from an independent cluster design, the $(i,j)$th entry of the covariance matrix $\Cov{\zv}$ is 1 if diversion units $i$ and $j$ are in the same cluster and $0$ otherwise.
Thus, by the observation above, this clustering objective is a correlation clustering where the weights are given by the matrix
\[
\Omega = \weightM^\tran \paren[\big]{\paren{1+\phi}\idM - \phi \onevec \onevec^\tran} \weightM \enspace.
\]
By inspection, we have that the $(i,j)$th entry of this matrix $\Omega$ is 
\[
\omega_{i,j} 
= \paren{1 + \phi} \sum_{k=1}^n w_{k,i} w_{k,j}
- \phi \paren[\Big]{\sum_{k=1}^n w_{k,i}} \paren[\Big]{\sum_{k=1}^n w_{k,j}} \enspace,
\]
as desired.
\end{proof}

\subsubsection{An instance of \exposuredesign when $\phi = 1/(n-1)$}\label{sec:prev_instance}

Now we demonstrate that the correlation clustering objective proposed in \cite{pouget2019variance} is a special case of \exposuredesign when $\phi = 1/(n-1)$.
Before giving the formal statement, we re-introduce the clustering objective in that paper; that is,
\begin{equation}\label{eq:exposure_spread_obj}\tag{\textsc{Exposure-Spread}\xspace}
\max_{\text{clusterings } \clustering} 
\Exp[\Bigg]{\sum_{i=1}^n \paren[\Bigg]{\dosei - \paren[\Big]{ \frac{1}{n} \sum_{j=1}^n \dosej} }^2}
\enspace,
\end{equation}
where the expectation is with respect to the treatment vector $\zv \in \setb{\pm 1}^m$ drawn according to the independent cluster design given by $\clustering$.
The quantity in the expectation is a measure of the spread of the exposures.
We remark that in \cite{pouget2019variance}, the exposures are called ``doses'' and the quantity in the expectation is referred to as the ``empirical dose variance''.

\begin{prop}\label{prop:more-general-clustering-obj}
Up to additive and multiplicative constants, \ref{eq:exposure_spread_obj} is equivalent to \exposuredesign when the trade-off parameter is set to $\phi = 1/(n-1)$.
\end{prop}

\begin{proof}
Let us denote the exposure spread by
\[
Q = \sum_{i=1}^n \paren[\Bigg]{\dosei - \paren[\Big]{ \frac{1}{n} \sum_{j=1}^n \dosej} }^2 \enspace,
\]
Note that the exposure spread is equal to the $\ell_2$ norm of the \emph{de-meaned} exposure vector $\bar{\dosev} = \paren{\bar{\dosee{1}}, \bar{\dosee{2}}, \dots \bar{\dosee{n}}}$, where
\[
\bar{\dosei} = \dosei - \paren[\Big]{ \frac{1}{n} \sum_{j=1}^n \dosej} \enspace .
\]
The entire de-meaned exposure vector may be written as $\bar{\dosev} = \paren{\idM - \frac{1}{n} \onevec \onevec^T} \dosev$.
Using the fact that this matrix is a projection and that the exposure vector is $\dosev = \weightM \zv$, we can write the exposure spread as 
\begin{align*}
Q
= \| \bar{\dosev} \|^2 
= \| \paren{\idM - \frac{1}{n} \onevec \onevec^T} \dosev \|^2 
= \dosev^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T}^2 \dosev 
= \dosev^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \dosev 
= \zv^\tran \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \zv \enspace.
\end{align*}
Finally, the expectation of the exposure spread may be written as
\begin{align*}
\Exp{Q}
&= \Exp[\Bigg]{ \zv^\tran \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \zv } 
    &\text{(from above)}\\
&= \Exp[\Bigg]{ \tr[\Big]{ \zv^\tran \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \zv }} 
    &\text{(trace of a scalar)}\\
&= \Exp[\Bigg]{ \tr[\Big]{ \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \zv \zv^\tran }} 
    &\text{(cyclic property of trace)}\\
&= \tr[\Big]{ \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \Exp{ \zv \zv^\tran }}
    &\text{(linearity of trace)} \\
&= \tr[\Big]{ \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \Cov{\zv}} + c \enspace,
\end{align*}
where the value $c$ in the last line is $c = \tr[\Big]{ \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \Exp{ \zv} \Exp{ \zv}^\tran }$, which follows from $\Cov{\zv} = \Exp{\zv \zv^\tran} - \Exp{\zv} \Exp{\zv}^\tran$ and linearity of trace.
Moreover, when the probability of treatment assignment $p$ is fixed, this value $c$ is a constant with respect to the clustering being chosen. 

Observe that by setting $\phi = 1/(n-1)$ and multiplying by a factor $(n-1)/n$, the \exposuredesign objective becomes
\[
\frac{n-1}{n} \tr[\Big]{ \weightM^\tran \paren[\big]{\paren{1+\frac{1}{n-1}}\idM - \frac{1}{n-1} \onevec \onevec^\tran} \weightM \Cov{\zv}}
=
\tr[\Big]{ \weightM^\tran \paren{\idM - \frac{1}{n} \onevec \onevec^T} \weightM \Cov{\zv}} \enspace.
\]
Thus, the \ref{eq:exposure_spread_obj} objective is equivalent (up to additive and multiplicative constants) to the \exposuredesign objective when $\phi = 1/(n-1)$.
\end{proof}

\subsubsection{Comparison to other correlation clustering variants}\label{sec:comparing_variants}

Recall that we defined the correlation clustering variant \corrclust as
$$
\max_{\substack{\text{partition } \\ \clustering \text{ of } \divunits}} 
\sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j} 
\enspace,
$$
where $\omega_{i,j}$ is defined for each pair of diversion units $i,j \in \divunits$ as
\begin{equation*} 
\omega_{i,j} 
= \paren{1 + \phi} \sum_{k=1}^n w_{k,i} w_{k,j}
- \phi \paren[\Big]{\sum_{k=1}^n w_{k,i}} \paren[\Big]{\sum_{k=1}^n w_{k,j}} \enspace,
\end{equation*}
and $w_{k,i}$ is the weight of the edge between the $k$th outcome unit and the $i$th diversion unit.
Observe that the term $\omega_{i,j}$ can take positive or negative values.

The maximization weighted correlation clustering variant considered by \cite{CGV05clustering, Swamy04correlation} is defined as follows. 
Let $G = (V,E)$ be a graph where each edge $e = (i,j) \in E$ has two \emph{non-negative} weights: $w_{in}(i,j)$ and $w_{out}(i,j)$.
Given a clustering $\clustering$, an edge $e = (i,j)$ is said to be \emph{in-cluster} if $i$ and $j$ are in the same cluster and \emph{out-cluster} otherwise.
The objective function for a given clustering is given by
\begin{equation}\tag{\corrclustCS}
    \sum_{\substack{\text{in-cluster} \\ \text{edges } e}} w_{in}(e) 
    + \sum_{\substack{\text{out-cluster} \\ \text{edges } e}} w_{out}(e)
\end{equation}
We now show that the \corrclust objective may be written as an instance of the \corrclustCS objective, but with the addition of a large additive constant.
Again, we stress that this reduction is primarily for aesthetic comparison purposes because the appearance of the large additive constant prevents any meaningful approximation-preserving reduction.

\begin{prop}
Our formulation \corrclust may be viewed as an instance of \corrclustCS with a large additive constant.
More precisely, let $w_{in}(i,j) = \max\{0, \omega_{i,j} \}$ and $w_{out}(i,j) = \min \{0, \omega_{i,j} \}$.
For a clustering $\clustering$, we have that the objectives are related by
\[
\sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j} 
- \sum_{i=1}^n \sum_{j=1}^n \min \{0, \omega_{i,j} \}
= \sum_{\substack{\text{in-cluster} \\ \text{edges } e}} w_{in}(e) 
    + \sum_{\substack{\text{out-cluster} \\ \text{edges } e}} w_{out}(e)
\]
\end{prop}
\begin{proof}
For each pair of diversion units $i,j$, define $\omega_{i,j}^+ = \max\{0, \omega_{i,j}\}$ and $\omega_{i,j}^- = -\min\{0, \omega_{i,j}\}$.
Observe that $\omega_{i,j} = \omega_{i,j}^+ + \omega_{i,j}^-$ and so we can re-distribute the following sum as
\[
\sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j} 
= \sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \paren[\Big]{\omega_{i,j}^+ + \omega_{i,j}^-}
= \sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j}^+
+ \sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j}^-
\enspace.
\]
Subtracting the (instance-dependent) constant $\sum_{i=1}^n \sum_{j=1}^n \min \{0, \omega_{i,j} \}$ from both sides and rearranging yields
\begin{align*}
\sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j}
    - \sum_{i=1}^n \sum_{j=1}^n \min \{0, \omega_{i,j} \}
&= \sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j}^+
    + \sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j}^-
    - \sum_{i=1}^n \sum_{j=1}^n \min \{0, \omega_{i,j} \} \\
&= \sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j}^+
    - \sum_{\cluste{r} \neq \cluste{r}' \in \clustering} \sum_{\substack{i \in \cluste{r} \\ j \in \cluste{r}'}} \omega_{i,j}^- \\
&= \sum_{\cluste{r} \in \clustering} \sum_{i, j \in \cluste{r}} \omega_{i,j}^+
    + \sum_{\cluste{r} \neq \cluste{r}' \in \clustering} \sum_{\substack{i \in \cluste{r} \\ j \in \cluste{r}'}} \paren{-\omega_{i,j}^-} \\
&= \sum_{\substack{\text{in-cluster} \\ \text{edges } e}} w_{in}(e) 
    + \sum_{\substack{\text{out-cluster} \\ \text{edges } e}} w_{out}(e) 
    \enspace.
\end{align*}
Finally, observe that for each pair $(i,j)$, the values $w_{in}(i,j)$  and $w_{out}(i,j)$ are non-negative so that the final equation is a valid objective function for the \corrclustCS formulation.
\end{proof}

